A unified framework of non-local parametric methods for image denoising

We propose a unified view of non-local methods for single-image denoising, for which BM3D is the most popular representative, that operate by gathering noisy patches together according to their similarities in order to process them collaboratively. Our general estimation framework is based on the minimization of the quadratic risk, which is approximated in two steps, and adapts to photon and electronic noises. Relying on unbiased risk estimation (URE) for the first step and on ``internal adaptation'', a concept borrowed from deep learning theory, for the second, we show that our approach enables to reinterpret and reconcile previous state-of-the-art non-local methods. Within this framework, we propose a novel denoiser called NL-Ridge that exploits linear combinations of patches. While conceptually simpler, we show that NL-Ridge can outperform well-established state-of-the-art single-image denoisers.

==> Tables/tableauPHOTOold.tex <==


\addtolength{\tabcolsep}{-5pt} 
\begin{figure}[t]
\centering
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{ccc}
 \begin{tikzpicture}
\node[anchor=south west,inner sep=0] (image) at (0,0)
  {\includegraphics[width=0.32\columnwidth]{./Figures/noisy09.png}};
\begin{scope}[x={(image.south east)},y={(image.north west)}]
  \begin{scope}[shift={(0,1)},x={(1/512,0)},y={(0,-1/512)}]
    \draw[dodgerblue, semithick] (110, 165) rectangle (155, 210);
    \draw[dodgerblue, thick] (287, 287) rectangle (512, 512);
    \draw[densely dashed, thin, dodgerblue] (110, 210) -> (287, 512);
    \draw[densely dashed, thin, dodgerblue] (155, 165) -> (512, 287);
  \end{scope}
\end{scope}
\end{tikzpicture}
&
\begin{tikzpicture}
\node[anchor=south west,inner sep=0] (image) at (0,0)
  {\includegraphics[width=0.32\columnwidth]{./Figures/bm3d09.png}};
\begin{scope}[x={(image.south east)},y={(image.north west)}]
  \begin{scope}[shift={(0,1)},x={(1/512,0)},y={(0,-1/512)}]
    \draw[dodgerblue, semithick] (110, 165) rectangle (155, 210);
    \draw[dodgerblue, thick] (287, 287) rectangle (512, 512);
    \draw[densely dashed, thin, dodgerblue] (110, 210) -> (287, 512);
    \draw[densely dashed, thin, dodgerblue] (155, 165) -> (512, 287);
  \end{scope}
\end{scope}
\end{tikzpicture}
& 
\begin{tikzpicture}
\node[anchor=south west,inner sep=0] (image) at (0,0)
  {\includegraphics[width=0.32\columnwidth]{./Figures/nlbayes09.png}};
\begin{scope}[x={(image.south east)},y={(image.north west)}]
  \begin{scope}[shift={(0,1)},x={(1/512,0)},y={(0,-1/512)}]
    \draw[dodgerblue, semithick] (110, 165) rectangle (155, 210);
    \draw[dodgerblue, thick] (287, 287) rectangle (512, 512);
    \draw[densely dashed, thin, dodgerblue] (110, 210) -> (287, 512);
    \draw[densely dashed, thin, dodgerblue] (155, 165) -> (512, 287);
  \end{scope}
\end{scope}
\end{tikzpicture}
\\
\footnotesize Noisy / 22.09 dB  &   \footnotesize BM3D \cite{BM3D} / 31.72 dB & \footnotesize NL-Bayes \cite{nlbayes} / 31.54 dB   \\
 \begin{tikzpicture}
\node[anchor=south west,inner sep=0] (image) at (0,0)
  {\includegraphics[width=0.32\columnwidth]{./Figures/s2s09.png}};
\begin{scope}[x={(image.south east)},y={(image.north west)}]
  \begin{scope}[shift={(0,1)},x={(1/512,0)},y={(0,-1/512)}]
    \draw[dodgerblue, semithick] (110, 165) rectangle (155, 210);
    \draw[dodgerblue, thick] (287, 287) rectangle (512, 512);
    \draw[densely dashed, thin, dodgerblue] (110, 210) -> (287, 512);
    \draw[densely dashed, thin, dodgerblue] (155, 165) -> (512, 287);
  \end{scope}
\end{scope}
\end{tikzpicture}
&
\begin{tikzpicture}
\node[anchor=south west,inner sep=0] (image) at (0,0)
  {\includegraphics[width=0.32\columnwidth]{./Figures/dncnn09.png}};
\begin{scope}[x={(image.south east)},y={(image.north west)}]
  \begin{scope}[shift={(0,1)},x={(1/512,0)},y={(0,-1/512)}]
    \draw[dodgerblue, semithick] (110, 165) rectangle (155, 210);
    \draw[dodgerblue, thick] (287, 287) rectangle (512, 512);
    \draw[densely dashed, thin, dodgerblue] (110, 210) -> (287, 512);
    \draw[densely dashed, thin, dodgerblue] (155, 165) -> (512, 287);
  \end{scope}
\end{scope}
\end{tikzpicture} 
&
\begin{tikzpicture}
\node[anchor=south west,inner sep=0] (image) at (0,0)
  {\includegraphics[width=0.32\columnwidth]{./Figures/nlridge09.png}};
\begin{scope}[x={(image.south east)},y={(image.north west)}]
  \begin{scope}[shift={(0,1)},x={(1/512,0)},y={(0,-1/512)}]
    \draw[dodgerblue, semithick] (110, 165) rectangle (155, 210);
    \draw[dodgerblue, thick] (287, 287) rectangle (512, 512);
    \draw[densely dashed, thin, dodgerblue] (110, 210) -> (287, 512);
    \draw[densely dashed, thin, dodgerblue] (155, 165) -> (512, 287);
  \end{scope}
\end{scope}
\end{tikzpicture} \\




\footnotesize Self2Self \cite{S2S} / 31.62 dB   &
\footnotesize DnCNN \cite{dncnn} / 31.06 dB  & \footnotesize NL-Ridge (ours) / \textbf{32.06} dB \\
\end{tabular}





\caption[Qualitative comparison of image denoising results with synthetic white Gaussian noise]{Denoising results (in PSNR) on \textit{Barbara} corrupted with additive white Gaussian noise ($\sigma = 20$).}
\label{nlridge_photo}
\end{figure}
\addtolength{\tabcolsep}{5pt}

==> Tables/tableauPSNR.tex <==

\afterpage{%
    \clearpage% Flush earlier floats (otherwise order might not be correct)
    \thispagestyle{empty}% empty page style (?)


\begin{landscape}


\begin{table*}
\centering
\caption[The PSNR results of different methods on datasets corrupted by Gaussian noise]{The PSNR (dB) results of different methods applied to three datasets corrupted with synthetic white Gaussian noise and $\sigma=5$, $15$, $25$, $35$ and $50$. The best method among each category (unsupervised or supervised) is emphasized in bold.}



\resizebox{\columnwidth}{!}{%
  \begin{NiceTabular}{|c@{\hspace{0.1cm}} c@{\hspace{0.1cm}} c l@{\hspace{0.5cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.7cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.7cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.0cm}} c|}
  \hline
 &&&  \multicolumn{1}{c}{\textbf{Methods}}
    & \multicolumn{9}{c}{\textbf{Set12}} & \multicolumn{9}{c}{\textbf{BSD68} \cite{berkeley}} & \multicolumn{9}{c}{\textbf{Urban100} \cite{urban}} & \\\hline\hline\noalign{\vskip 0.1cm}

   &&& Noisy & 34.25 &/&  24.61 &/& 20.17 &/&  17.25 &/& 14.15 & 34.25 &/& 24.61 &/& 20.17 &/&  17.25 &/&  14.15 &  34.25 &/& 24.61 &/& 20.17 &/&  17.25 &/& 14.15 & \\[0.1cm]
   \hline\noalign{\vskip 0.1cm}

 \multirow{10}{*}{\begin{sideways} \small \textbf{Unsupervised} \end{sideways}} & \multirow{6}{*}{\begin{sideways} \small \textit{Traditional} \end{sideways}} && BM3D \cite{BM3D}  &  38.02 &/& 32.37 &/& 29.97 &/& 28.40 &/& 26.72 &  37.55 &/& 31.07 &/& 28.57 &/& 27.08 &/& 25.62 & 38.30 &/& 32.35  &/& 29.70 &/& 27.97 &/&  25.95 &\\
 &&& NL-Bayes \cite{nlbayes} &  38.12 &/&  32.25 &/& 29.88 &/& 28.30 &/&  26.45 & 37.62 &/& 31.16 &/& \bf{28.70} &/&  \bf{27.18} &/&  25.58 & 38.33 &/& 31.96 &/& 29.34  &/& 27.61 &/& 25.56 &\\
 

 
 %&&& \textbf{NL-Ridge} (linear)  &   \bf{38.19} &/& \bf{32.46} &/& \bf{30.00} &/& \bf{28.41} &/& \bf{26.73} &  \bf{37.67} &/& \bf{31.20} &/& 28.67 &/& 27.14 &/& \bf{25.67} & \bf{38.56} &/& \bf{32.53} &/& \bf{29.90} &/& \bf{28.13} &/& \bf{26.29} &\\
 \cdashline{4-32}\noalign{\vskip 0.1cm} 
 
 &&& \textbf{NL-Ridge} \textit{(linear)}  &   \bf{38.19} &/& \bf{32.46} &/& 30.00 &/& 28.41 &/& 26.73 &  \bf{37.67} &/& \bf{31.20} &/& 28.67 &/& 27.14 &/& 25.67 & \bf{38.56} &/& 32.53 &/& 29.90 &/& 28.13 &/& 26.29 &\\

 &&&  \textbf{NL-Ridge} \textit{(affine)}  &   38.17 &/& 32.42 &/& 29.98 &/& \bf{28.43} &/& \bf{26.79} &  37.65 &/& 31.18 &/& 28.68 &/& 27.16 &/& \bf{25.71} & 38.54 &/& \bf{32.54} &/& \bf{29.93} &/& \textbf{28.21} &/& \bf{26.40} &\\


  &&&  \textbf{NL-Ridge} \textit{(conical)}  &   38.03 &/& 32.16 &/& 29.72 &/& 28.07 &/& 26.49 & 37.46 &/& 30.86 &/& 28.38 &/& 26.85 &/& 25.43 &- &/& - &/& - &/& - &/& - &\\

 &&& \textbf{NL-Ridge} \textit{(convex)}  &   38.00 &/& 32.14 &/& 29.70 &/& 28.14 &/& 26.51 &  37.45 &/& 30.85 &/& 28.38 &/& 26.86 &/& 25.44 & -\iffalse 38.30 \fi &/& - &/& - &/& - &/& - &\\[0.1cm]


\cdashline{2-32}\noalign{\vskip 0.1cm}

 & \multirow{3}{*}{\begin{sideways} \small \textit{Deep} \end{sideways}} & \multirow{3}{*}{\begin{sideways} \small \textit{learning} \end{sideways}} & DIP \cite{DIP}  &  -  &/&  30.12  &/& 27.54 &/& - &/& 24.67  &  - &/& 28.83 &/& 26.59 &/& - &/& 24.13  & - &/& - &/& -  &/& - &/& - &\\
 &&& Noise2Self \cite{N2S}    &  - &/& 31.01 &/& 28.64 &/& - &/& 25.30 & - &/&  29.46 &/& 27.72 &/& - &/& 24.77  & - &/& - &/& -  &/& - &/& - &\\

 &&& Self2Self \cite{S2S}   &  - &/& 32.07 &/& \bf{30.02} &/& - &/& 26.49 &  - &/& 30.62  &/& 28.60 &/& -&/&  25.70 & - &/& - &/& -  &/& - &/& - &\\[0.1cm] 
 
 \hline\noalign{\vskip 0.1cm}

   \multirow{4}{*}{\begin{sideways} \small \textbf{Supervised} \end{sideways}} &&& DnCNN \cite{dncnn} &  - &/& \bf{\bf{32.86}} &/& \bf{\bf{30.44}} &/& 28.82 &/& 27.18 & - &/& \bf{\bf{31.73}} &/& \bf{\bf{29.23}} &/& 27.69  &/& 26.23 & - &/& 32.68 &/& 29.97 &/& 28.11 &/& 26.28  & \\
 &&& FFDNet \cite{ffdnet} &  \bf{\bf{38.11}} &/& 32.75 &/& 30.43 &/& \bf{\bf{28.92}} &/& \bf{\bf{27.32}} & \bf{\bf{37.80}} &/& 31.63 &/& 29.19 &/& \bf{\bf{27.73}}  &/& \bf{\bf{26.29}} &  \bf{\bf{38.12}} &/& 32.43 &/& 29.92 &/& \bf{\bf{28.27}} &/& \bf{\bf{26.52}} & \\
 &&& LIDIA \cite{LIDIA} &  - &/& 32.85 &/& 30.41 &/& -&/&  27.19 & - &/& 31.62 &/& 29.11 &/& -&/&  26.17 & - &/& \bf{\bf{32.80}} &/& \bf{\bf{30.12}} &/& - &/& 26.51 & \\
 &&& DCT2net \cite{dct2net} &  37.65 &/& 32.10 &/& 29.71 &/& 28.10 &/&  26.39 & 37.34 &/& 31.09 &/& 28.64 &/& 27.17 &/&  25.68 & 37.59 &/& 31.48 &/& 28.81 &/& 27.04 &/& 25.17 & \\[0.1cm] \hline
\end{NiceTabular}%
}


\label{nlridge_resultsPSNR00}
\end{table*}






\begin{table*}[!t]
\centering
  \caption[The PSNR results of different methods on Darmstadt Noise Dataset (DND)]{The PSNR (dB) results on raw data on Darmstadt Noise Dataset (DND) \cite{DND}}
\resizebox{0.9\columnwidth}{!}{%
  \begin{NiceTabular}{*{10}{|c}|} \hline 
  &  \multicolumn{5}{c}{\textit{Unsupervised}} & \multicolumn{4}{c}{\textit{Supervised}} \\\hline
  \textbf{Methods} & BM3D \cite{BM3D} &  \textbf{NL-Ridge}  & KSVD \cite{ksvd} & NCSR  \cite{NCSR}  & WNNM \cite{WNNM}    & MLP \cite{mlp} & TNRD \cite{tnrd}  & FFDNet \cite{ffdnet} & DCT2net \cite{dct2net}    \\\hline\hline
  \textbf{PSNR (in dB)} & \textbf{47.15}  &  47.12  & 46.87 & 47.07    & 47.05   & 45.71  & 45.70  & \textbf{47.40} & 46.83  \\\hline
\end{NiceTabular}%
}
\label{nlrigde_dnd_res}
\end{table*}


\end{landscape}
\clearpage% Flush page
}








==> tableau2.tex <==


